kHGCN: Tree-likeness Modeling via Continuous and Discrete Curvature Learning

The prevalence of tree-like structures, encompassing hierarchical structures and power law distributions, exists extensively in real-world applications, including recommendation systems, ecosystems, financial networks, social networks, etc. Recently, the exploitation of hyperbolic space for tree-likeness modeling has garnered considerable attention owing to its exponential growth volume. Compared to the flat Euclidean space, the curved hyperbolic space provides a more amenable and embeddable room, especially for datasets exhibiting implicit tree-like architectures. However, the intricate nature of real-world tree-like data presents a considerable challenge, as it frequently displays a heterogeneous composition of tree-like, flat, and circular regions. The direct embedding of such heterogeneous structures into a homogeneous embedding space (i.e., hyperbolic space) inevitably leads to heavy distortions. To mitigate the aforementioned shortage, this study endeavors to explore the curvature between discrete structure and continuous learning space, aiming at encoding the message conveyed by the network topology in the learning process, thereby improving tree-likeness modeling. To the end, a curvature-aware hyperbolic graph convolutional neural network, \{kappa}HGCN, is proposed, which utilizes the curvature to guide message passing and improve long-range propagation. Extensive experiments on node classification and link prediction tasks verify the superiority of the proposal as it consistently outperforms various competitive models by a large margin.

==> computation_of_orc.tex <==
\section{Computation of ORC}
\label{appendix:computation_orc}
Here, we give one derivation  of Ollivier-Ricci curvature  for the reader's convenience. % on the reformulation. 
First, the theorem of Kantorovich duality is borrowed to approximate the opposite direction of Definition~\ref{def:curvature}.

\begin{theorem}[Kantorovich duality.] Let $G(V, E)$ be a locally finite graph, and let $m_1, m_2$ be two probability measures, then
\begin{equation}
\begin{aligned}
    W(m_1, m_2)=\sup_{\phi\in f_{1-lip}}\left\{ \sum_{v_i\in V}\phi(v_i)m_1(v_i)-\sum_{v_j\in V}\phi(v_j)m_2(v_j)\right\},
\end{aligned}
\end{equation}
\end{theorem}
where $f_{1-lip}$ denotes the 1-Lipschitz functions. With finite support $v_i$ and $v_j$, we can rewrite it as the standard form of a linear programming problem:
\begin{equation}
\label{equ:15}
W(m_1, m_2)=\sup_{S\phi\leq d}m\cdot \phi.
\end{equation}
Here $\phi$, $m$ and $d$ are column vectors,
$$
\phi:=(\phi(v_i)..., \phi(v_n), -\phi(v_j), ..., -\phi(v_m))^T\in \mathbb{R}^{(n+m)},
$$
$$
s:=(m_1(v_i)..., m_1(v_n), m_2(v_j), ..., m2(v_m))^T\in \mathbb{R}^{(n+m)},
$$
let $d_g^*(u, v)$ be the shortest graph distance between $u$ and $v$, then
\begin{equation*}
\begin{aligned}
            d:=(d_g^*(v_1, u_1),...,d_g^*(v_1, u_m),...,d_g^*(v_n, u_1),\\
            ..., d_g^*(v_n, u_m))^T\in \mathbb{R}^{nm},
\end{aligned}
\end{equation*}
and $S$ is defined as a $nm\times nm$ matrix which consists of $m\times n$ matrix $m_i$ and $m\times m$ identity matrix $I_i$ $(i\in[1,n])$, that is 
$$
S:=\left(\begin{array}{cc}
s_{1} & I_1 \\
\vdots & \vdots \\
s_{n} & I_n
\end{array}\right),
$$
where $s_i$ is a matrix that the elements in column $i$ equal to $1$ and the elements in other columns are zero, for example:
$$
s_{1}=\left(\begin{array}{cccc}
1 & 0 & \cdots & 0 \\
\vdots & \vdots & \ddots & \vdots \\
1 & 0 & \cdots & 0
\end{array}\right).
$$

With the reformulation as Equation~(\ref{equ:15}), the ORC is relatively simple to calculate numerically via the SciPy module in Python. The computation cost is reported in Table~\ref{tab:curvature_computing}. 
 It is worth noting that the self-loop edges need to be removed when calculating the Ricci curvature to ensure  $G=(V, E)$ a locally finite, connected and simple graph. While the edges of the self-loop play an indispensable role in regularization and preventing over-smoothing. Therefore, we further add the self-loop and assign the Ricci curvature value to zero after finishing the calculation of the curvature, which indicates that we treat the self-loop as a local ``flat'' connection.

